A Distributed Model-Free Algorithm for Multi-hop Ride-sharing using Deep Reinforcement Learning

The growth of autonomous vehicles, ridesharing systems, and self driving technology will bring a shift in the way ride hailing platforms plan out their services. However, these advances in technology coupled with road congestion, environmental concerns, fuel usage, vehicles emissions, and the high cost of the vehicle usage have brought more attention to better utilize the use of vehicles and their capacities. In this paper, we propose a novel multi-hop ride-sharing (MHRS) algorithm that uses deep reinforcement learning to learn optimal vehicle dispatch and matching decisions by interacting with the external environment. By allowing customers to transfer between vehicles, i.e., ride with one vehicle for sometime and then transfer to another one, MHRS helps in attaining 30\% lower cost and 20\% more efficient utilization of fleets, as compared to the ride-sharing algorithms. This flexibility of multi-hop feature gives a seamless experience to customers and ride-sharing companies, and thus improves ride-sharing services.

==> new_figs_v3/accept_rate_vehicle_num_v3.tex <==
% This file was created by tikzplotlib v0.8.4.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={white!69.01960784313725!black},
xlabel={No of Vehicles},
xmajorgrids,
xmin=4800, xmax=9200,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Accept Rate},
ymajorgrids,
ymin=0.917099009013976, ymax=0.980920810706508,
ytick style={color=black}
]
\addplot [very thick, green!50.19607843137255!black, mark=*, mark size=6, mark options={solid}]
table {%
5000 0.955999092093317
6000 0.975119802691333
7000 0.975189802691333
8000 0.975190038386263
9000 0.978019819720484
};
\addlegendentry{MHRS}
\addplot [very thick, red, dashed, mark=triangle*, mark size=6, mark options={solid,rotate=180}]
table {%
5000 0.93
6000 0.935
7000 0.945
8000 0.95
9000 0.955
};
\addlegendentry{DeepPool}
\addplot [very thick, blue, dashed, mark=square*, mark size=6, mark options={solid}]
table {%
5000 0.92
6000 0.921
7000 0.925
8000 0.949
9000 0.955
};
\addlegendentry{MOVI}
\end{axis}

\end{tikzpicture}

==> test.tex <==
\begin{figure*}[h]
\begin{minipage}[b]{1.0\linewidth}
    \centering
    \subfigure[$K=1$]{
        \input{accept_rate_num_hops_v3.tex}
        \caption{Accept rate versus the average number of hops.}
        \label{accept_vs_hop}
        %\label{fig:fig_1}
    }
    \subfigure[$K=2$]{
        \input{effective_distance_num_hops_v3.tex}
        \caption{Effective distance ratio versus number of hops.}
		\label{Effdist_vs_hops}
    }
    \subfigure[$K=3$]{
        \input{idle_time_accept_rate_v3.tex}
        \caption{Average idle time per request for different accept rate.}
		\label{idle_vs_accept}
    }
\end{minipage}
\caption{Caption loda lasun}
\label{fig:final_fig}
\end{figure*}
